Makespan Scheduling of Unit Jobs with Precedence Constraints in $O(1.995^n)$ time

In a classical scheduling problem, we are given a set of $n$ jobs of unit length along with precedence constraints and the goal is to find a schedule of these jobs on $m$ identical machines that minimizes the makespan. This problem is well-known to be NP-hard for an unbounded number of machines. Using standard 3-field notation, it is known as $P|\text{prec}, p_j=1|C_{\max}$. We present an algorithm for this problem that runs in $O(1.995^n)$ time. Before our work, even for $m=3$ machines the best known algorithms ran in $O^\ast(2^n)$ time. In contrast, our algorithm works when the number of machines $m$ is unbounded. A crucial ingredient of our approach is an algorithm with a runtime that is only single-exponential in the vertex cover of the comparability graph of the precedence constraint graph. This heavily relies on insights from a classical result by Dolev and Warmuth (Journal of Algorithms 1984) for precedence graphs without long chains.

==> Makefile <==
all: main.pdf

main.pdf: main.tex references.bib main.bbl
	pdflatex main.tex
	pdflatex main.tex

main.aux: $(SOURCES)
	pdflatex main.tex

main.bbl: references.bib main.aux
	bibtex main

clean:
	rm -f img/*.log img/*.aux
	rm -f *~ *.log *.out *.aux *.blg *.bbl *.gz

distclean: clean
	rm -f main.pdf

tar: clean
	bash -c "cd ..; tar -czf ${BASE}.tar.gz ${BASE}/*; mv ${BASE}.tar.gz ${BASE}"

spell:
	@for i in `find . -name "*.tex"` ; do \
		echo "------------ $$i --------------" ; \
		aspell list --lang=en --mode=tex --dont-tex-check-comments --personal=./blue-slownik.txt < $$i | sort | uniq ; \
done

diff:
	mkdir /tmp/cut-and-count-diff/
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d2.tex
	git checkout $(branch-id)
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d1.tex
	latexdiff /tmp/cut-and-count-diff/d1.tex /tmp/cut-and-count-diff/d2.tex > /tmp/cut-and-count-diff/diff.tex
	pdflatex /tmp/cut-and-count-diff/diff.tex
	git checkout master


==> scratchpad.tex <==

schedule(G,S,T) // checks if G[pred(T) \cap succ(S)] has a tight 3-schedule
If |S| \geq \sqrt{n} AND |T| \geq \sqrt{n}
(WRONG: If |S| \geq \sqrt{n} OR |T| \geq \sqrt{n})
branch on a sink moment ($n^3$ branches, we reduce with $\sqrt{n}$ vertices in both branches (BUT this assumes many sources AND many sinks) so we get $n^{O(\sqrt{n})}$ run time

